Learning Algorithm Hyperparameters for Fast Parametric Convex Optimization

We introduce a machine-learning framework to learn the hyperparameter sequence of first-order methods (e.g., the step sizes in gradient descent) to quickly solve parametric convex optimization problems. Our computational architecture amounts to running fixed-point iterations where the hyperparameters are the same across all parametric instances and consists of two phases. In the first step-varying phase the hyperparameters vary across iterations, while in the second steady-state phase the hyperparameters are constant across iterations. Our learned optimizer is flexible in that it can be evaluated on any number of iterations and is guaranteed to converge to an optimal solution. To train, we minimize the mean square error to a ground truth solution. In the case of gradient descent, the one-step optimal step size is the solution to a least squares problem, and in the case of unconstrained quadratic minimization, we can compute the two and three-step optimal solutions in closed-form. In other cases, we backpropagate through the algorithm steps to minimize the training objective after a given number of steps. We show how to learn hyperparameters for several popular algorithms: gradient descent, proximal gradient descent, and two ADMM-based solvers: OSQP and SCS. We use a sample convergence bound to obtain generalization guarantees for the performance of our learned algorithm for unseen data, providing both lower and upper bounds. We showcase the effectiveness of our method with many examples, including ones from control, signal processing, and machine learning. Remarkably, our approach is highly data-efficient in that we only use $10$ problem instances to train the hyperparameters in all of our examples.

==> cover/simods_coverletter.tex <==
% !TeX root = simods_coverletter.tex
% !TEX program = pdflatex
\input{simods_coverletter_preamble}

\begin{document}
\hfill{\today}

SIAM Journal on the Mathematics of Data Science

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Learning Algorithm Hyperparameters for Fast Parametric Convex Optimization}'' to the \emph{SIAM Journal on the Mathematics of Data Science}.
% Our manuscript studies \red{X, Y, and Z} which is important because of \red{A, B, and C}.
Our manuscript introduces a \red{machine-learning framework to learn the hyperparameter sequence of first-order methods for convex optimization} which is important because many \red{applications require real-time solutions to these problems}.
Our computational architecture amounts to running fixed-point iterations where the algorithm hyperparameters are shared across problem instances.
We first allow the hyperparameters to vary across iterations, but, after a predefined number of steps, we force them to be constant. %from this point onwards.
We guarantee convergence for our method and use a sample convergence bound with a validation dataset to obtain generalization guarantees to unseen problem instances.
% Up until a predefined number of iterations, we allow these hyperparameters to vary, but after some point we force them to be constant from here on out.
We optimize the hyperparameters by minimizing the mean square error to ground truth solutions over a set of training instances.
We apply our learning framework to numerous examples in control, statistics, and signal processing, and show that our method significantly reduces the number of iterations needed to obtain high-quality solutions.
Moreover, we show that our approach is highly data-efficient since we only use ten training instances in each of our examples.

% Our architecture consists of a neural network mapping problem parameters to warm starts, followed by a predefined number of fixed-point iterations.
% In this way, the neural network predicts warm-starts with the end-to-end goal of minimizing the downstream loss.
% Theoretically, we obtain PAC-Bayes generalization bounds to unseen data.
% We apply our learning framework to numerous examples in control, statistics, and signal processing, observing significantly reduced solution times.



% Our manuscript introduces a \red{data-driven approach to analyze the performance of continuous algorithms for parametric optimization} which is important because many \red{worst-case analyses for classical optimizers can be too pessimistic} and \red{learned optimizers lack strong generalization guarantees}.
% We use statistical learning theory, namely a sample convergence bound and PAC-Bayes theory, to provide guarantees for both classical and learned optimizers.
% We apply our methods to numerous examples in control, signal processing, and meta-learning.
% For classical optimizers, our bounds are much tighter than
% those that worst-case guarantees provide. 
% For learned optimizers, our bounds outperform the empirical outcomes observed in their non-learned counterparts.

% Our architecture consists of a neural network mapping problem parameters to warm starts, followed by a predefined number of fixed-point iterations.
% In this way, the neural network predicts warm-starts with the end-to-end goal of minimizing the downstream loss.
% We apply our methods to numerous examples in control, statistics, and signal processing, observing significantly reduced solution times.



We suggest the following action editors and referees for our submission.

Section Editor:
\begin{itemize}
    \item \red{Alexandre d'Aspremont}, Ecole Normale Superieure (aspremon@ens.fr)
\end{itemize}

Action Editors:
\begin{itemize}
    \item \red{Madeleine Udell}, Stanford University (udell@stanford.edu)
    \item \red{Steve Wright}, University of Wisconsin-Madison (swright@cs.wisc.edu)
    \item \red{Coralia Cartis}, Oxford University (Coralia.Cartis@maths.ox.ac.uk)
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{Joe Marino}, Google DeepMind (josephmarino@google.com)
    \item \red{Atlas Wang}, University of Texas, Austin (atlaswang@utexas.edu)
    \item \red{Ernest Ryu}, University of California, Los Angeles (eryu@math.ucla.edu)
    \item \red{Yisong Yue}, California Institute of Technology (yyue@caltech.edu)
    \item \red{Pontus Giselsson}, Lund University (pontusg@control.lth.se)
    \item \red{Soheil Kolouri}, Vanderbilt University (soheil.kolouri@vanderbilt.edu)
\end{itemize}

% Our submission has the following keywords: \red{learning to optimize}, \red{statistical learning theory}, \red{generalization bounds}, \red{fixed-point iterations}, \red{parametric optimization}.

% As the corresponding author, I confirm that the co-author listed below does not have a conflict of interest with the editors and referees I suggest above. 
% Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{SIAM Journal on the Mathematics of Data Science}.
As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. 
Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{SIAM Journal on the Mathematics of Data Science}.


\bigskip

Sincerely,

\medskip

Rajiv Sambharya (University of Pennsylvania)\\
Bartolomeo Stellato (Princeton University)

\end{document}







































